Understanding and Characterizing Mock Assertions in Unit Tests

Mock assertions provide developers with a powerful means to validate program behaviors that are unobservable to test assertions. Despite their significance, they are rarely considered by automated test generation techniques. Effective generation of mock assertions requires understanding how they are used in practice. Although previous studies highlighted the importance of mock assertions, none provide insight into their usages. To bridge this gap, we conducted the first empirical study on mock assertions, examining their adoption, the characteristics of the verified method invocations, and their effectiveness in fault detection. Our analysis of 4,652 test cases from 11 popular Java projects reveals that mock assertions are mostly applied to validating specific kinds of method calls, such as those interacting with external resources and those reflecting whether a certain code path was traversed in systems under test. Additionally, we find that mock assertions complement traditional test assertions by ensuring the desired side effects have been produced, validating control flow logic, and checking internal computation results. Our findings contribute to a better understanding of mock assertion usages and provide a foundation for future related research such as automated test generation that support mock assertions.

==> acmart-preload-hook.tex <==
% \PassOptionsToPackage{bookmarks=false}{hyperref}

